SPVR: syntax-to-prompt vulnerability repair based on large language models

Purpose: In the field of vulnerability repair, previous research has leveraged pretrained models and LLM-based prompt engineering, among which LLM-based approaches show better generalizability and achieve the best performance. However, the LLM-based approaches generally regard vulnerability repair as a sequence-to-sequence task, and do not explicitly capture the syntax patterns for different vulnerability types, leading to limited accuracy. We aim to create a method that ensures the specificity of prompts targeting vulnerable code while also leveraging the generative capabilities of Large Language Models. Methods: We propose SPVR (Syntax-to-Prompt Vulnerability Repair), a novel framework that collects information from syntax trees, and generates corresponding prompts. Our method consists of three steps: rule design, prompt generation, and patch generation. In the rule design step, our method parses code patches and designs rules to extract relevant contextual information. These rules aid in identifying vulnerability-related issues. In the prompt generation step, our method extracts information from vulnerable code with pre-defined rules, automatically converting them into prompts. We also incorporate the description of CWE (Common Weakness Enumeration) as known information into the prompts. Finally, in the patch generation step, this prompt will serve as input to any conversational LLM to obtain code patches. Results: Extensive experiments validate that our method achieves excellent results in assisting LLMs to fix vulnerabilities accurately. We utilize multiple Large Language Models to validate the effectiveness of our work, repairing 143 of 547 vulnerable code using ChatGPT-4. We conducted a comparison of our approach against several existing vulnerability repair approaches (including fine-tuning-based and prompt-based), across multiple metrics.

==> spvr/00-abstract-new.tex <==

% \begin{abstract}
% In the field of vulnerability repair, previous research has leveraged pre-trained models and LLM-based prompt engineering, among which LLM-based approaches show better generalizability and achieve the best performance. However, the LLM-based approaches generally regard vulnerability repair as a sequence-to-sequence task, and do not explicitly capture the syntax patterns for different vulnerability types, leading to limited accuracy. Automatically integrating the syntax information into LLMs is challenging since syntax patterns for different vulnerability types tend to be disparate and are hard to be defined.


% To address the challenge, we propose \tool (Syntax-to-Prompt Vulnerability Repair), a novel framework that collects information from syntax trees, and generates corresponding prompts.
% \tool consists of three steps: Rule design, prompt generation, and patch generation.
% In the rule design step, \tool parses code patches and designs rules to extract relevant contextual information. These rules aid in identifying vulnerability-related issues.
% In the prompt generation step, \tool extracts necessary information from vulnerable code with pre-defined rules, automatically converting them into prompts. We also incorporate the description of CWE (Common Weakness Enumeration) as known information into the prompts.
% Finally, in the patch generation step, this prompt will serve as input to any conversational LLM to obtain code patches.
% Notably, our framework is independent of any specific LLMs. Extensive experiments validate that \tool achieves excellent results in assisting LLMs to fix vulnerabilities accurately. We utilize multiple large language models to validate the effectiveness of our work, achieving a 26\% higher accuracy compared to an existing LLM-based vulnerability repair method. We believe our approach has promising application prospects for enhancing real-world code security.
% \end{abstract}



% \begin{abstract}
% \textit{Context:}
% In the field of vulnerability repair, previous research has leveraged pre-trained models and LLM-based prompt engineering, among which LLM-based approaches show better generalizability and achieve the best performance. However, the LLM-based approaches generally regard vulnerability repair as a sequence-to-sequence task, and do not explicitly capture the syntax patterns for different vulnerability types, leading to limited accuracy. 

% \noindent
% \textit{Objectives:}
% We aim to create a method that ensures the specificity of prompts targeting vulnerable code while also leveraging the generative capabilities of Large Language Models.

% \noindent
% \textit{Methods:}
% We propose SPVR (Syntax-to-Prompt Vulnerability Repair), a novel framework that collects information from syntax trees, and generates corresponding prompts. Our method consists of three steps: Rule design, prompt generation, and patch generation. In the rule design step, our method parses code patches and designs rules to extract relevant contextual information. These rules aid in identifying vulnerability-related issues. In the prompt generation step, our method extracts necessary information from vulnerable code with pre-defined rules, automatically converting them into prompts. We also incorporate the description of CWE (Common Weakness Enumeration) as known information into the prompts. Finally, in the patch generation step, this prompt will serve as input to any conversational LLM to obtain code patches.

% \noindent
% \textit{Results:}
% Extensive experiments validate that our method achieves excellent results in assisting LLMs to fix vulnerabilities accurately. We utilize multiple large language models to validate the effectiveness of our work, repairing 143 of 547 vulnerable code using ChatGPT-4. We conducted a comparison of our approach against several existing vulnerability repair approaches (including fine-tuning based and prompt-based), across multiple metrics. 

% \noindent
% \textit{Conclusion:}
% Our method is a novel framework that combines the AST structure of code, providing targeted prompts of repair code for vulnerabilities. We believe it has promising application prospects for real-world code vulnerability repair.


% \end{abstract}
